Monadic Second-Order Logic with Arbitrary Monadic Predicates

We study Monadic Second-Order Logic (MSO) over finite words, extended with (non-uniform arbitrary) monadic predicates. We show that it defines a class of languages that has algebraic, automata-theoretic and machine-independent characterizations. We consider the regularity question: given a language in this class, when is it regular? To answer this, we show a substitution property and the existence of a syntactical predicate. We give three applications. The first two are to give very simple proofs that the Straubing Conjecture holds for all fragments of MSO with monadic predicates, and that the Crane Beach Conjecture holds for MSO with monadic predicates. The third is to show that it is decidable whether a language defined by an MSO formula with morphic predicates is regular.

==> advice_regular_predicates.tex <==

The advice regular predicates are defined by MSO formulae over a one-letter alphabet.

\begin{definition}[Advice regular predicates]
A $k$-ary predicate $\bold{P} = (\bold{P}_n)_{n \in \N}$ is advice regular 
if there exists a formula $\varphi(\liste{Q},\liste{x}) \in \MSO[\leq,\NN_1]({a}^*)$ 
and predicates $\liste{\bold{Q}} \in \NN_1$ such that 
$$\bold{P}_n = \set{\liste{\bold{x}} \in \set{0,n-1}^k \mid\ 
a^n,\liste{\bold{Q}},\liste{\bold{x}} \models \varphi}.$$ 
We denote by $\M$ the class of advice regular predicates,
and by $\MU$ the class of uniform advice regular predicates.
\end{definition}

\begin{example}\label{ex:areg}
The following predicates are advice regular:
\begin{itemize}
	\item all regular predicates,
	\item the uniform predicate 
\[
\set{(x,y)\mid 
\begin{array}{c} \text{ the number of prime numbers } \\ \text{between x and y is even}\end{array}
},
\]
	\item the non-uniform predicate
\[
(\set{(x,y) \mid \exists z, x < z < y \text{ and } n \text{ is a power of }z})_{n \in \N}.
\]
\end{itemize}
\end{example}

We now give two characterizations of advice regular languages,
will be used for two purposes: proving that some predicates are not advice regular,
and proving the Crane Beach Property for advice regular languages in Section~\ref{sec:crane_beach}.

\begin{definition}[Myhill-Nerode equivalence relations]
Given $L \subseteq A^*$ and $p \in \N$, we define two equivalence relations:
\begin{itemize}
	\item $u \sim_L v$ if for all $w \in A^*$, we have $$u w \in L \Longleftrightarrow v w \in L,$$
	\item $u \sim_{L,p} v$ if for all $w \in A^p$, we have $$u w \in L \Longleftrightarrow v w \in L.$$
\end{itemize}
The relation $\sim_L$ is called the Myhill-Nerode equivalence relation,
and the second is a coarser relation, which we call the $p$-Myhill-Nerode equivalence relation.
\end{definition}

Recall that $\sim_L$ contains finitely many equivalence classes if and only if $L$ is regular,
\textit{i.e.} $L \in \MSO[\le]$.

\begin{definition}[Automata with non-uniform advice]
A non-deterministic automaton with non-uniform advice is given by $\A = (Q,q_0,\delta,F)$
where $Q$ is a finite set of states, $q_0 \in Q$ is the initial state, 
$\delta \subseteq \N \times \N \times Q \times A \times Q$ is the transition relation
and $F \subseteq \N \times Q$ is the set of final states.
In the deterministic case $\delta : \N \times \N \times Q \times A \rightarrow Q$.

A run over a finite word $w = w_0 \cdots w_{n-1} \in A^*$ is a finite word $\rho = q_0 \cdots q_n \in Q^*$
such that for all $i \in \set{0,\ldots,n-1}$, we have $(i,n,q_i,w_i,q_{i+1}) \in \delta$.
It is accepting if $(n,q_n) \in F$.
\end{definition}

Automata with non-uniform advice are (much) more expressive than classical automata
since they have access to two more pieces of informations about the word being read: its length and the current position.
Both the transitions and the final states can depend on those two informations.

\begin{example}\label{ex:aut}
The language $\set{a^n b^n c^n \mid n \text{ is a prime number}}$ 
is recognized by a (deterministic) automaton with non-uniform advice.

The automaton has five states, $q_a,q_b,q_c,q_F$ and $\bot$. The initial state is $q_a$.
The transition function is defined as follows:
$$\begin{array}{llll}
\delta(3n,i,q_a,a) & = & q_a & \textrm{ if } i < n-1 \\
\delta(3n,n-1,q_a,a) & = & q_b \\
\delta(3n,i,q_b,b) & = & q_b & \textrm{ if } n \le i < 2n-1 \\
\delta(3n,2n-1,q_b,c) & = & q_c \\
\delta(3n,i,q_c,c) & = & q_c & \textrm{ if } 2n \le i < 3n-1 \\
\delta(3n,3n-1,q_c,c) & = & q_F \\
\end{array}$$
All other transitions lead to $\bot$, the sink rejecting state.
The set of final states is $F = \set{(3n,q_F) \mid n \text{ is a prime number}}$.
The automaton is represented in figure~\ref{fig:aut}.
\input{aut}
\end{example}

\begin{theorem}[Regular languages with monadic predicates]\label{thm:regular_languages_non_uniform_predicates}
Let $L \subseteq A^*$, the following properties are equivalent:
\begin{enumerate}
	\item[(1)] $L \in \MSO[\le,\NN_1](A^*)$,
	\item[(2)] $L$ is recognized by a non-deterministic automaton with non-uniform advice,
	\item[(3)] $L$ is recognized by a deterministic automaton with non-uniform advice,
	\item[(4)] There exists $K \in \N$ such that for all $n,p \in \N$, 
	the restriction of $\sim_{L,p}$ to words of length $n$ contains at most $K$ equivalence classes.
\end{enumerate}
In such case, we say that $L$ is advice regular.
\end{theorem}

%This theorem extends the Myhill-Nerode theorem proposed in~\cite{KRSZ12},
%as they only work with monadic uniform predicates (called advice).

We sketch the proof, explaining the following implications: $2 \Rightarrow 1$, then $2 \Rightarrow 3$, then $3 \Rightarrow 2$, 
then $1 \Rightarrow 2$, 
then $3 \Rightarrow 4$ and finally $4 \Rightarrow 3$.

The implication $2 \Rightarrow 1$ amounts to write a formula checking for the existence of a run.
Let $\A = (Q,q_0,\delta,F)$ be a non-deterministic automaton with non-uniform advice,
where $Q = \set{0,\ldots,\ell-1}$ and $q_0 = 0$.
First, let $X^0,\ldots,X^{\ell-1}$ be a $\ell$-tuple of monadic second-order variables.
We first need to express that $\liste{X}$ partitions the set of all positions of the word.
This is easily expressed by the following formula, denoted $\chi(\liste{X})$:
\[
\forall x,\ \left(\bigvee_i x \in X_i\right)\ \wedge\ \bigvee_i
\left(x \in X_i\to \bigwedge_{j \neq i} x \notin X_j\right)\ .
\]

For each $q \in Q$, we define the uniform predicate $\bold{P}^q$ by $\bold{P}^q = \set{n \in \N \mid (n,q) \in F}$.
The formula in figure~\ref{form:3} checks for the existence of an accepting run,
and uses the monadic predicates $\bold{P}^q$ for $q \in Q$, $\textrm{first}$ (the first position of the word),
$\textrm{last}$ (the last position of the word) and $\textrm{length}$ (the length of the word).
\begin{figure*}[!t]
\normalsize
\begin{equation*}
\exists X^0,\ldots,X^{\ell-1},\
\begin{cases}
\qquad \chi(\liste{X}) \\
\wedge\ \forall x, \textrm{first}(x) \Longrightarrow x \in X_0 \\
\wedge\ \forall x, \forall n, \neg \textrm{last}(x) \wedge \textrm{last}(n) \Longrightarrow\ \bigvee_{(x,n,q,a,q') \in \delta}\quad 
X_q(x) \wedge a(x) \wedge X_{q'}(x+1) \\
\wedge\ \forall x, \textrm{last}(x) \Longrightarrow \bigvee_{q \in Q} x \in X_q \wedge x \in \bold{P}^q\ .
\end{cases}
\end{equation*}
\hrulefill
\caption{Formula checking for the existence of an accepting run.\label{form:3}}
\end{figure*}

The implication $2 \Rightarrow 3$ consists in determinizing automata with non-uniform advice,
extending the classical powerset construction.
Let $\A = (Q,q_0,\delta,F)$ be a non-deterministic automaton with non-uniform advice,
we construct the deterministic automaton with non-uniform advice $\A' = (Q',\set{q_0},\delta',F')$,
where $Q'$ is the powerset of $Q$, the set of final states is 
$F' = \set{(n,S) \mid \exists q \in S, (n,q) \in F}$, and the transition function $\delta'$ is defined by:
\[
\delta'(i,n,S,a) = \set{q' \in Q \mid \exists q \in S, (i,n,q,a,q') \in \delta}\ .
\]
It is easy to see that $\A$ and $\A'$ are equivalent.

The implication $3 \Rightarrow 2$ is immediate from the definitions.

The implication $1 \Rightarrow 2$ requires us to show closure properties of automata with non-uniform advice 
under union, projection and complementation.
The first two closures are obtained in the exact same way as in the classical case, we do not detail them here; 
for the third case, we rely on the equivalence between $2$ and $3$,
and complement deterministic (complete) automata with non-uniform advice
by simply exchanging $F$ and its complement in $\N \times Q$.

For the implication $3 \Rightarrow 4$, let $\A$ be a deterministic automaton with non-uniform advice,
and consider the mapping $t_{n,p} : A^n \rightarrow Q$ defined for $w = w_0 \cdots w_{n-1}$ by
$t_{n,p}(w) = \delta(n,n',\delta(n-1,n',\cdots \delta(0,n',q_0,w_0) \cdots, w_{n-2}), w_{n-1})$,
for $n' = n+p$.
In words, $t_{n,p}(w)$ is the state reached by $\A$ while reading $w$ assuming that the total word will be of length $n+p$.
We argue that $t_{n,p}(w) = t_{n,p}(w')$ implies $w \sim_{L,p} w'$: indeed, for $u \in A^p$, after reading $w$ or $w'$,
the automaton $\A$ is in the same state, so it will either accept both $wu$ and $w'u$ or reject both.
Note that $t_{n,p}$ can have at most $|Q|$ different values.
Consequently, the restriction of $\sim_{L,p}$ to words of length $n$ contains at most $|Q|$ equivalence classes.

We now prove the implication $4 \Rightarrow 3$, by constructing a deterministic automaton with non-uniform advice.
Its set of states is $Q = \set{1,\ldots,K}$.
To each word $w$ and length $p \ge 0$ we associate $\lfloor w \rfloor_p \in Q$ such that 
if $w$ and $w'$ have the same length, then $w \sim_{L,p} w'$ if and only if $\lfloor w \rfloor_p = \lfloor w' \rfloor_p$.
We set $\lfloor \varepsilon \rfloor_p = 1$ for all $p$; the initial state is $1$.
The transition function is defined by $\delta(n,n+p,\lfloor w \rfloor_p,a) = \lfloor wa \rfloor_{p-1}$,
for \textit{some} $w$ of length $n$. 
(This is well defined: if $\lfloor w \rfloor_p = \lfloor w' \rfloor_p$, then $w \sim_{L,p} w'$,
so $wa \sim_{L,p-1} w'a$, thus $\lfloor wa \rfloor_{p-1} = \lfloor w'a \rfloor_{p-1}$.)
The set of final states is $$F = \set{(n,\lfloor w \rfloor_0) \mid w \in A^n \cap L}.$$
We argue that this automaton recognizes $L$:
whenever it reads $w = w_0 \cdots w_{n-1}$, the corresponding run is
$$\rho = \lfloor \varepsilon \rfloor_n \lfloor w_0 \rfloor_{n-1} \lfloor w_0 w_1 \rfloor_{n-2} \cdots 
\lfloor w_0 \cdots w_{n-1} \rfloor_0,$$
which is accepting if and only if $w \in L$.


\begin{corollary}[Advice regular predicates]\label{cor:advice_regular_predicates}
Let $\bold{P} = (\bold{P}_n)_{n \in \N}$ be a $k$-ary predicate,
define 
\[
L_\bold{P} = \set{u \in \set{0,1}^k \mid 
\begin{array}{c} 
u \text{ has length } n \ \wedge \\ 
\bold{P}_n = \set{(x_1,\ldots,x_k) \mid u_i(x_i) = 1}
\end{array}}.
\]
The following properties are equivalent:
\begin{enumerate}
	\item[(1)] $\bold{P}$ is advice regular,
	\item[(2)] $L_\bold{P}$ is recognized by a deterministic automaton with non-uniform advice,
	\item[(3)] There exists $K \in \N$ such that for all $n,p \in \N$, 
	the restriction of $\sim_{L_\bold{P},p}$ to words of length $n$ contains at most $K$ equivalence classes.
\end{enumerate}
\end{corollary}

We can use Corollary~\ref{cor:advice_regular_predicates} to prove that some predicates are not advice regular.

\begin{fact}
The uniform predicate $\bold{P} = \set{(x,y) \mid y = 2 \cdot x}$ is not advice regular.
\end{fact}

\begin{proof}
We show that $L_\bold{P}$ does not satisfy the property $(3)$.
Fix $K$, and consider the words
\[
u^i = 
\binom{0}{0}^{2K-1-i} 
\binom{1}{0}
\binom{0}{0}^{K+i} 
\]
for $i \in \set{0,\ldots,\frac{K-1}{2}}$.
They all have length $3K$.
Observe that for $i \neq j$, $u^i \not\sim_{L_\bold{P},K} u^j$,
since for the words
\[
v^i = 
\binom{0}{0}^{K-1-2i} 
\binom{0}{1}
\binom{0}{0}^{2i} 
\]
which are all of length $K$, we have $u^i \cdot v^j \in L_\bold{P}$ if and only if $i = j$.
\end{proof}

Note that this implies that neither the $+$ nor the $\times$ predicates are advice regular.

